Schottky barriers, emission regimes and contact resistances in 2H-1T' MoS$_2$ lateral metal-semiconductor junctions from first-principles

We have studied the finite bias transport properties of a 2H-1T' MoS$_2$ lateral metal-semiconductor (M-S) junction by non-equilibrium Green's functions calculations, aimed at contacting the 2D channel in a field effect transistor. Our results indicate that (a) despite the fundamentally different electrostatics of line and planar dipoles, the Schottky barrier heights respond similarly to changes in doping and applied bias in 2D and 3D M-S junctions, (b) 2H-1T' MoS$_2$ lateral junctions are free from Fermi level pinning, (c) armchair interfaces have superior contacting properties vs.\ zigzag interfaces, (d) 1T' contacts to $p$ channels will present a reduced contact resistance by a factor of 4-10 with respect to $n$ channels and (e) contacts to intermediately doped $n$ ($p$) channels operate in the field (thermionic) emission regime. We also provide an improved procedure to experimentally determine the emission regime in 2D material junctions.

==> xx.tex <==


